Real-time 6-DoF Pose Estimation by an Event-based Camera using Active LED Markers

Real-time applications for autonomous operations depend largely on fast and robust vision-based localization systems. Since image processing tasks require processing large amounts of data, the computational resources often limit the performance of other processes. To overcome this limitation, traditional marker-based localization systems are widely used since they are easy to integrate and achieve reliable accuracy. However, classical marker-based localization systems significantly depend on standard cameras with low frame rates, which often lack accuracy due to motion blur. In contrast, event-based cameras provide high temporal resolution and a high dynamic range, which can be utilized for fast localization tasks, even under challenging visual conditions. This paper proposes a simple but effective event-based pose estimation system using active LED markers (ALM) for fast and accurate pose estimation. The proposed algorithm is able to operate in real time with a latency below \SI{0.5}{\milli\second} while maintaining output rates of \SI{3}{\kilo \hertz}. Experimental results in static and dynamic scenarios are presented to demonstrate the performance of the proposed approach in terms of computational speed and absolute accuracy, using the OptiTrack system as the basis for measurement.

==> graphics/bias/packages.tex <==
\usepackage{xcolor}
\usepackage{siunitx}
% \sisetup{per-mode=symbol,binary-units=true,exponent-product = \cdot}

%\usepackage[nohyperlinks]{acronym}

\usepackage{tikz}


==> graphics/bias/packages_pgfplots.tex <==
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}
\pgfkeys{/pgf/number format/.cd,1000 sep={\,}}
\pgfplotsset{compat=1.12,height=0.3\textheight,legend cell align=left,tick scale binop=\times}
\pgfplotsset{tick style={black,thin}}
\pgfplotsset{every axis plot/.append style={line width=0.8pt}}
% \pgfplotsset{every axis/.append style={line join=round,no markers}}
\pgfplotsset{every axis/.append style={line join=round}}
% \pgfplotsset{legend style={draw=none,fill=white,fill opacity=0.6,text opacity=1}}
\pgfplotsset{ylabsh/.style={every axis y label/.style={at={(0,0.5)}, xshift=#1, rotate=90}}}
\pgfplotsset{
  legend image with text/.style={
    legend image code/.code={%
      \node[anchor=center] at (0.3cm,0cm) {#1};
    }
  },
}

% \pgfplotsset{
%   cycle list={acin_red,thick\\
%     acin_green_variant,thick\\
%     TU_blue,thick\\
%     TU_violet_variant!80!black,thick\\
%     orange!90!white,thick\\
%     acin_green!45!TU_blue!90,thick\\
%     TU_gray,thick\\
%     brown!80!black,thick\\
%   }
% }

\pgfplotsset{
    colormap={parula}{
        rgb255=(53,42,135)
        rgb255=(15,92,221)
        rgb255=(18,125,216)
        rgb255=(7,156,207)
        rgb255=(21,177,180)
        rgb255=(89,189,140)
        rgb255=(165,190,107)
        rgb255=(225,185,82)
        rgb255=(252,206,46)
        rgb255=(249,251,14)
    },
}


==> graphics/colors.tex <==
% Definition eines einheitlichen Farbschemas und Definition von styles.
%=======================================================================

% Um ein einheitliches Farbschema zu gewährleisten werden hier einige Farben und
% davon abgeleitete Variationen definiert. Diese Farben werden in der Vorlage
% bereits für die entsprechenden Befehle (Links, Hervorhebung, usw.) verwendet.
% Die Farben sollten auch in Grafiken verwendet werden. Die RGB- bzw. CMYK Codes
% werden hierzu in der Dokumentation angegeben.
% Es werden außerdem einige styles hier definiert, die von verschiedenen
% Befehlen verwendet werden.


% Definition der Grundfarben
%============================

\definecolor{acin_red}{RGB}{186, 18, 43}
\definecolor{acin_gray}{RGB}{176, 176, 176}
\definecolor{acin_yellow}{RGB}{252, 204, 71}
\definecolor{acin_green}{RGB}{0, 190, 65}
\definecolor{TU_blue}{RGB}{0, 102, 153}
\definecolor{test2}{rgb}{0,0.47,0.85}
\definecolor{TU_gray}{RGB}{102, 102, 102}
\providecolor{test}{rgb}{0.85, 0, 0.22}

\definecolor{acin_red_complement}{RGB}{50,255,0}
\definecolor{TU_blue_complement}{RGB}{255,106,0}
\definecolor{acin_yellow_variant}{RGB}{255,238,0}
\definecolor{acin_green_variant}{RGB}{25,150,0}
\definecolor{acin_blue_variant}{RGB}{19,93,255}
\definecolor{TU_green_variant}{RGB}{157,217,0}
\definecolor{TU_pink_variant}{RGB}{202,0,90}
\definecolor{TU_violet_variant}{RGB}{218,33,255}

% Definition von abgeleiteten Farben
%====================================

\colorlet{acin_red_lightvar}{acin_red!80}
\colorlet{acin_red_verylightvar}{acin_red!25!white!97!acin_gray}
\colorlet{TU_blue_light}{TU_blue!30!white}

% Alternative Namen
%===================
\definecolor{red}{named}{acin_red}
\definecolor{gray}{named}{TU_gray}
\definecolor{yellow}{named}{acin_yellow}
\definecolor{green}{named}{acin_green}
\definecolor{blue}{named}{TU_blue}

\definecolor{light_red}{named}{acin_red_lightvar}


\definecolor{emph}{named}{acin_red} % Farbe für Hervorhebungen
\definecolor{env}{named}{TU_blue} % Farbe für Umgebungen
\definecolor{env_bck}{RGB}{235,235,235} % Hintergrundfarbe für Umgebungen
\definecolor{link_color}{named}{TU_blue} % Links
\definecolor{url_color}{named}{TU_blue} % urls
\definecolor{cite_color}{named}{acin_green} % Zitate

\definecolor{HinweisGreen}{named}{acin_green_variant}
\colorlet{HinweisGreen_bck}{HinweisGreen!15!white}
\definecolor{HinweisYellow}{RGB}{250, 170,	40}
\colorlet{HinweisYellow_bck}{HinweisYellow!10!white}
\definecolor{HinweisBlue}{named}{TU_blue}
\colorlet{HinweisBlue_bck}{HinweisBlue!25!white}
\colorlet{HinweisBW}{black!60!white}
\colorlet{HinweisBW_bck}{HinweisBW!15!white}

\definecolor{EditorNote}{named}{orange}
\colorlet{EditorNote_bck}{EditorNote!25!white}

\colorlet{eqn}{TU_blue!70!black!15!white}
\colorlet{eqn_bck}{TU_blue!70!black!15!white}

\colorlet{proof}{TU_blue!70!black!15!white}

\definecolor{EqnEmph1}{named}{acin_yellow}
\colorlet{EqnEmph2}{TU_blue!70!black!15!white}
\definecolor{EqnEmph3}{named}{acin_red_verylightvar}

\colorlet{table_rule_inner}{black!30!white}


==> graphics/macros.tex <==
\newcommand*{\fullref}[1]{\cref{#1} \hyperref[{#1}]{``\nameref*{#1}''}} % One single link

\providecommand{\wrt}{w.\,r.\,t.\@\xspace} 
\providecommand{\etal}{et\ al.\@\xspace} 

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\inv}[1]{{#1}^{-1}}
\newcommand{\numsetR}{\mathds{R}}
\newcommand{\numsetN}{\mathds{N}}
\newcommand{\normII}[1]{\norm{#1}}
\newcommand{\normInf}[1]{\norm{#1}_\infty}
\newcommand{\zero}{\vec 0}
\newcommand{\identity}{\vec I}
\newcommand{\ubar}[1]{\text{\b{$#1$}}}
\renewcommand{\d}{^{\mathrm d}}
\newcommand{\DiffC}[1]{\frac{\mathrm{D}}{\dd #1}}
\newcommand{\SOIII}{\mathrm{SO(3)}}

\renewcommand{\natural}{_{\mathrm n}}
\renewcommand{\parallel}{_{\mathrm p}}

\newcommand{\Frame}[1]{{\mathcal{#1}}}
\newcommand{\FrameWorld}{\Frame{W}}
\newcommand{\FrameBase}{\Frame{B}}
\newcommand{\FrameEndeffector}{\Frame{E}}
\newcommand{\FrameTool}{\Frame{T}}
\newcommand{\FramePlanar}{\Frame{A}}
\newcommand{\FrameContact}{\Frame{C}}
\newcommand{\FrameObject}{\Frame{O}}
\newcommand{\FrameTriangle}[1]{\Frame{T}_{#1}}
\newcommand{\FrameTrianglei}{\Frame{T}_i}
\newcommand{\FrameContactNatural}{\Frame{C}\natural}
\newcommand{\FrameContactParallel}{\Frame{C}\parallel}
\newcommand{\FrameContactParallelTilde}{\tilde{\Frame{C}}\parallel}
\newcommand{\EulContactNatural}{\vec c\natural}
\newcommand{\EulContactParallel}{\vec c\parallel}
\newcommand{\FrameLink}{\Frame{L}}

\newcommand{\Hom}[2]{\vec H_{#1}^{#2}}
\newcommand{\Rot}[2]{\vec R_{#1}^{#2}}
\newcommand{\Rotp}[2]{\dot{\vec R}_{#1}^{#2}}
\newcommand{\Tran}[2]{\vec d_{#1}^{#2}}
\newcommand{\HomTran}[2]{\vec H_{\mathrm T#1,#2}}
\newcommand{\HomRot}[2]{\vec H_{\mathrm R#1,#2}}
\newcommand{\Roti}[2]{\vec R_{#1\mathrm,#2}}
\newcommand{\Skew}[1]{\vec S\left(#1\right)}
\newcommand{\Unskew}[1]{\inv{\vec S}\left(#1\right)}
\newcommand{\Eul}{\vec \phi}
\newcommand{\Eulp}{\dot{\vec \phi}}
\newcommand{\Eult}{\tilde{\vec \phi}}
\newcommand{\ProjectionMatrix}{\vec A}
\newcommand{\EulAng}{\phi}
\newcommand{\EulAngI}{\EulAng_1}
\newcommand{\EulAngIp}{\dot{\EulAng}_1}
\newcommand{\EulAngII}{\EulAng_2}
\newcommand{\EulAngIIp}{\dot{\EulAng}_2}
\newcommand{\EulAngIII}{\EulAng_3}
\newcommand{\EulAngIIIp}{\dot{\EulAng}_3}
\newcommand{\EulT}{\vec T}
\newcommand{\AngVel}[2]{\vec \omega_{#1}^{#2}}
\newcommand{\AngAcc}[2]{\dot{\vec \omega}_{#1}^{#2}}
\newcommand{\Q}{Q}
\newcommand{\Qtilde}{\tilde{Q}}
\newcommand{\X}{X_6}
\newcommand{\rr}{r_\mathrm{r}}

\newcommand{\Mcomp}{\vec \Lambda}
\newcommand{\Ccomp}{\vec \Gamma}
\renewcommand{\t}{\vec \theta}
\newcommand{\tp}{\dot{\vec \theta}}
\newcommand{\tpk}{\dot{\vec \theta}_k}
\newcommand{\thpk}{\dot{\hat{\vec \theta}}_k}
\newcommand{\thpkI}{\dot{\hat{\vec \theta}}_{k+1}}
\newcommand{\tpp}{\ddot{\vec \theta}}
\newcommand{\Mlink}{\M_\mathrm l}
\newcommand{\Mrotor}{\M_\mathrm r}
\newcommand{\Mcoup}{\vec U}
\newcommand{\B}{\vec B}
\newcommand{\qt}{\tilde{\q}}
\newcommand{\qtp}{\dot{\qt}}
\newcommand{\qtpp}{\ddot{\qt}}

\newcommand{\q}{\vec q}
\newcommand{\qI}{q_1}
\newcommand{\qII}{q_2}
\newcommand{\qIII}{q_3}
\newcommand{\qIV}{q_4}
\newcommand{\qV}{q_5}
\newcommand{\qVI}{q_6}
\newcommand{\qVII}{q_7}
\renewcommand{\z}{\vec z}
\newcommand{\qb}{\bar{\vec q}}
\newcommand{\qp}{\dot{\vec q}}
\newcommand{\qpb}{\dot{\bar{\vec q}}}
\newcommand{\qpp}{\ddot{\vec q}}
\newcommand{\qppb}{\ddot{\bar{\vec q}}}
\newcommand{\qs}{\vec q_0^*}
\newcommand{\M}{\vec M}
\newcommand{\Mb}{\vec{\bar{M}}}
\newcommand{\n}{\vec n}
\newcommand{\C}{\vec C}
\newcommand{\g}{\vec g}
\newcommand{\K}{\vec K}
\newcommand{\D}{\vec D}
\newcommand{\taum}{{\vec\tau}_{\mathrm{m}}}
\newcommand{\taumk}{{\vec\tau}_{\mathrm{m},k}}
\renewcommand{\u}{\vec u}
\newcommand{\uI}{u_1}
\newcommand{\uII}{u_2}
\newcommand{\uIII}{u_3}
\newcommand{\uIV}{u_4}
\newcommand{\uV}{u_5}
\newcommand{\uVI}{u_6}
\newcommand{\uVII}{u_7}
\newcommand{\taumI}{{\tau}_{\mathrm{m,1}}}
\newcommand{\taumII}{{\tau}_{\mathrm{m,2}}}
\newcommand{\taumIII}{{\tau}_{\mathrm{m,3}}}
\newcommand{\taumIV}{{\tau}_{\mathrm{m,4}}}
\newcommand{\taumV}{{\tau}_{\mathrm{m,5}}}
\newcommand{\taumVI}{{\tau}_{\mathrm{m,6}}}
\newcommand{\taumVII}{{\tau}_{\mathrm{m,7}}}
\newcommand{\taun}{{\vec\tau}_{\mathrm{n}}}
\newcommand{\taunI}{{\vec\tau}_{\mathrm{n,1}}}
\newcommand{\taunII}{{\vec\tau}_{\mathrm{n,2}}}
\newcommand{\tauc}{{\vec\tau}_{\mathrm{c}}}
\newcommand{\tauj}{\vec\tau}
\newcommand{\taujp}{\dot{\tauj}}
\newcommand{\taue}{{{\vec\tau}_{\mathrm{e}}}}
\newcommand{\taueb}{{\bar{\vec\tau}_{\mathrm{e}}}}
\newcommand{\tauf}{{{\vec\tau}_{\mathrm{f}}}}
\newcommand{\taufhk}{{\hat{\vec\tau}_{\mathrm{f},k}}}
\newcommand{\FrictionObserverParameter}{F}
\newcommand{\FrictionObserverMatrix}{\vec \FrictionObserverParameter}
\newcommand{\V}{\vec v}
\newcommand{\vd}{\vec v\d}
\newcommand{\vt}{\vec v_\mathrm t}
\newcommand{\vr}{\vec v_\mathrm r}
\newcommand{\vtilde}{\tilde{\vec v}}

\renewcommand{\y}{\vec y}
\newcommand{\yp}{\dot{\vec y}}
\newcommand{\ypp}{\ddot{\vec y}}
\newcommand{\yt}{{\vec y}_\mathrm t}
\newcommand{\Yt}{Y_\mathrm t}
\newcommand{\ytp}{\dot{\vec y}_\mathrm t}
\newcommand{\yr}{{\vec y}_\mathrm r}
\newcommand{\yrp}{\dot{\vec y}_\mathrm r}

%y hat
\newcommand{\yh}{\hat{\vec y}}
\newcommand{\yhI}{\hat{y}_1}
\newcommand{\yhII}{\hat{y}_2}
\newcommand{\yhIII}{\hat{y}_3}
\newcommand{\yhIV}{\hat{y}_4}
\newcommand{\yhV}{\hat{y}_5}
\newcommand{\yhVI}{\hat{y}_6}
%y hat punkt
\newcommand{\yhp}{\dot{\hat{\vec y}}}
\newcommand{\yhpI}{\dot{\hat{y}}_1}
\newcommand{\yhpII}{\dot{\hat{y}}_2}
\newcommand{\yhpIII}{\dot{\hat{y}}_3}
\newcommand{\yhpIV}{\dot{\hat{y}}_4}
\newcommand{\yhpV}{\dot{\hat{y}}_5}
\newcommand{\yhpVI}{\dot{\hat{y}}_6}
%y hat punkt punkt
\newcommand{\yhpp}{\ddot{\hat{\vec y}}}
\newcommand{\yhppI}{\ddot{\hat{y}}_1}
\newcommand{\yhppII}{\ddot{\hat{y}}_2}
\newcommand{\yhppIII}{\ddot{\hat{y}}_3}
\newcommand{\yhppIV}{\ddot{\hat{y}}_4}
\newcommand{\yhppV}{\ddot{\hat{y}}_5}
\newcommand{\yhppVI}{\ddot{\hat{y}}_6}
%y hat desired
\newcommand{\yhd}{\hat{\vec y}\d}
\newcommand{\yhdI}{\hat{y}_1\d}
\newcommand{\yhdII}{\hat{y}_2\d}
\newcommand{\yhdIII}{\hat{y}_3\d}
\newcommand{\yhdIV}{\hat{y}_4\d}
\newcommand{\yhdV}{\hat{y}_5\d}
\newcommand{\yhdVI}{\hat{y}_6\d}
%y hat desired punkt
\newcommand{\yhdp}{\dot{\hat{\vec y}}\d}
\newcommand{\yhdpI}{\dot{\hat{y}}_1\d}
\newcommand{\yhdpII}{\dot{\hat{y}}_2\d}
\newcommand{\yhdpIII}{\dot{\hat{y}}_3\d}
\newcommand{\yhdpIV}{\dot{\hat{y}}_4\d}
\newcommand{\yhdpV}{\dot{\hat{y}}_5\d}
\newcommand{\yhdpVI}{\dot{\hat{y}}_6\d}
%y hat desired punkt punkt
\newcommand{\yhdpp}{\ddot{\hat{\vec y}}\d}
\newcommand{\yhdppI}{\ddot{\hat{y}}\d_1}
\newcommand{\yhdppII}{\ddot{\hat{y}}\d_2}
\newcommand{\yhdppIII}{\ddot{\hat{y}}\d_3}
\newcommand{\yhdppIV}{\ddot{\hat{y}}\d_4}
\newcommand{\yhdppV}{\ddot{\hat{y}}\d_5}
\newcommand{\yhdppVI}{\ddot{\hat{y}}\d_6}
%y hat position
\newcommand{\yhP}{\hat{\vec y}^\mathrm p}
\newcommand{\yhPp}{\dot{\hat{\vec y}}^\mathrm p}
\newcommand{\yhPpp}{\ddot{\hat{\vec y}}^\mathrm p}
%y tilde
\newcommand{\ytilde}{\tilde{\vec y}}
\newcommand{\ytildep}{\dot{\tilde{\vec y}}}
\newcommand{\ytildepp}{\ddot{\tilde{\vec y}}}
%y tilde desired
\newcommand{\ytilded}{\tilde{\vec y}\d}
\newcommand{\ytildedp}{\dot{\tilde{\vec y}}\d}
\newcommand{\ytildedpp}{\ddot{\tilde{\vec y}}\d}
%e hat
\newcommand{\eh}{\hat{\vec e}}
\newcommand{\eht}{\hat{\vec e}_\mathrm t}
\newcommand{\ehtp}{\dot{\hat{\vec e}}_\mathrm t}
\newcommand{\ehtpp}{\ddot{\hat{\vec e}}_\mathrm t}
\newcommand{\ehr}{\hat{\vec e}_\mathrm r}
\newcommand{\ehI}{\hat{e}_1}
\newcommand{\ehII}{\hat{e}_2}
\newcommand{\ehIII}{\hat{e}_3}
\newcommand{\ehIV}{\hat{e}_4}
\newcommand{\ehV}{\hat{e}_5}
\newcommand{\ehVI}{\hat{e}_6}
%e hat punkt
\newcommand{\ehp}{\dot{\hat{\vec e}}}
%e hat punkt punkt
\newcommand{\ehpp}{\ddot{\hat{\vec e}}}
%e hat force
\newcommand{\ehF}{\hat{\vec e}_\mathrm f}
%e hat force punkt
\newcommand{\ehFp}{\dot{\hat{\vec e}}_\mathrm f}
%e tilde
\newcommand{\etilde}{\tilde{\vec e}}
\newcommand{\etildeI}{\tilde{e}_1}
\newcommand{\etildeII}{\tilde{e}_2}
\newcommand{\etildeIII}{\tilde{e}_3}
\newcommand{\etildeIV}{\tilde{e}_4}
\newcommand{\etildeV}{\tilde{e}_5}
\newcommand{\etildeVI}{\tilde{e}_6}

\renewcommand{\H}{\vec h}
\newcommand{\Ht}{{\vec h}_\mathrm t}
\newcommand{\Hr}{{\vec h}_\mathrm r}
\newcommand{\Jg}{\vec J_\mathrm g}
\newcommand{\Ja}{\vec J}
\newcommand{\Jt}{\vec J_\mathrm t}
\newcommand{\Jr}{\vec J_\mathrm r}
\newcommand{\Jp}{\dot{\vec J}}
\newcommand{\Jh}{\hat{\vec J}}
\newcommand{\Jht}{\hat{\vec J}_\mathrm t}
\newcommand{\Jhr}{\hat{\vec J}_\mathrm r}
\newcommand{\JhreI}{\hat{\vec j}_{\mathrm r,\eI}}
\newcommand{\JhreII}{\hat{\vec j}_{\mathrm r,\eII}}
\newcommand{\JhreIII}{\hat{\vec j}_{\mathrm r,\eIII}}
\newcommand{\Jhrei}{\hat{\vec j}_{\mathrm r,\ei}}
\newcommand{\Jhrer}{\hat{\vec j}_{\mathrm r,\er}}
\newcommand{\Jhp}{\dot{\hat{\vec J}}}
\newcommand{\Jtilde}{\tilde{\Ja}}
\newcommand{\Jtildep}{\dot{\tilde{\Ja}}}
\newcommand{\Proj}{\mathrm{P}}
\newcommand{\ProjNatural}{\mathrm{P}_\mathrm{n}}
\newcommand{\ProjParallel}{\mathrm{P}_\mathrm{p}}

\newcommand{\fe}{\vec f_\mathrm e}
\newcommand{\feh}{\hat{\vec f}_\mathrm e}
%See https://tex.stackexchange.com/a/59740
\newcommand{\fehp}{\dot{\hat{\vec f\hspace{0pt}}}_\mathrm e}
\newcommand{\fehd}{\hat{\vec f}_\mathrm e\d}
%See https://tex.stackexchange.com/a/59740
\newcommand{\fehdp}{\dot{\hat{\vec f\hspace{0pt}}}_\mathrm e\d}
\newcommand{\fehI}{\hat{f}_{\mathrm e,1}}
\newcommand{\fehII}{\hat{f}_{\mathrm e,2}}
\newcommand{\fehIII}{\hat{f}_{\mathrm e,3}}
\newcommand{\fehIV}{\hat{f}_{\mathrm e,4}}
\newcommand{\fehV}{\hat{f}_{\mathrm e,5}}
\newcommand{\fehVI}{\hat{f}_{\mathrm e,6}}
\newcommand{\fehdI}{\hat{f}_{\mathrm e,1}\d}
\newcommand{\fehdII}{\hat{f}_{\mathrm e,2}\d}
\newcommand{\fehdIII}{\hat{f}_{\mathrm e,3}\d}
\newcommand{\fehdIV}{\hat{f}_{\mathrm e,4}\d}
\newcommand{\fehdV}{\hat{f}_{\mathrm e,5}\d}
\newcommand{\fehdVI}{\hat{f}_{\mathrm e,6}\d}
\newcommand{\fehIp}{\dot{\hat{f}}_{\mathrm e,1}}
\newcommand{\fehIIp}{\dot{\hat{f}}_{\mathrm e,2}}
\newcommand{\fehIIIp}{\dot{\hat{f}}_{\mathrm e,3}}
\newcommand{\fehIVp}{\dot{\hat{f}}_{\mathrm e,4}}
\newcommand{\fehVp}{\dot{\hat{f}}_{\mathrm e,5}}
\newcommand{\fehVIp}{\dot{\hat{f}}_{\mathrm e,6}}
\newcommand{\fehdIp}{\dot{\hat{f}}_{\mathrm e,1}\d}
\newcommand{\fehdIIp}{\dot{\hat{f}}_{\mathrm e,2}\d}
\newcommand{\fehdIIIp}{\dot{\hat{f}}_{\mathrm e,3}\d}
\newcommand{\fehdIVp}{\dot{\hat{f}}_{\mathrm e,4}\d}
\newcommand{\fehdVp}{\dot{\hat{f}}_{\mathrm e,5}\d}
\newcommand{\fehdVIp}{\dot{\hat{f}}_{\mathrm e,6}\d}
\newcommand{\Md}{\vec M\d}
\newcommand{\md}{m\d}
\newcommand{\mdi}{m\d_i}
\newcommand{\mdI}{m\d_1}
\newcommand{\mdII}{m\d_2}
\newcommand{\mdIII}{m\d_3}
\newcommand{\mdIV}{m\d_4}
\newcommand{\mdV}{m\d_5}
\newcommand{\mdVI}{m\d_6}
\newcommand{\Dd}{\vec D\d}
\newcommand{\ddd}{d\d}
\newcommand{\Kd}{\vec K\d}
\newcommand{\kd}{k\d}

\newcommand{\Dn}{\vec D_\mathrm n}
\newcommand{\Kn}{\vec K_\mathrm n}

%Path
\renewcommand{\P}{\pi}
\newcommand{\p}{\vec \P}
\newcommand{\pp}{p}
\newcommand{\pps}{p^*}
\newcommand{\ppt}{P_\mathrm t}
\newcommand{\ppsk}{p^*_k}
\newcommand{\ppsp}{\dot{p}^*}
\newcommand{\pt}{\vec \pi_\mathrm p}
\newcommand{\ps}{\pi_\mathrm l}
\newcommand{\pspp}{\ddot{\pi}_\mathrm l}
\newcommand{\pg}{\pi_\mathrm g}
\newcommand{\pgi}{\pi_{\mathrm{g,}i}}
\newcommand{\tI}{t_1}
\newcommand{\tII}{t_2}

%Surface
\renewcommand{\S}{\sigma}
\newcommand{\s}{\vec \S}
\newcommand{\sn}{\vec \S_\mathrm{n}}
\renewcommand{\sp}{\vec s}
\newcommand{\spi}{s_i}
\newcommand{\spj}{s_j}
\newcommand{\spI}{s_1}
\newcommand{\spIz}{s_{1,0}}
\newcommand{\spII}{s_2}
\newcommand{\spIIz}{s_{2,0}}
\newcommand{\sspi}{\s_{s_i}}
\newcommand{\sspI}{\s_{s_1}}
\newcommand{\sspIspI}{\s_{s_1s_1}}
\newcommand{\sspIspII}{\s_{s_1s_2}}
\newcommand{\sspII}{\s_{s_2}}
\newcommand{\sspIIspI}{\s_{s_2s_1}}
\newcommand{\sspIIspII}{\s_{s_2s_2}}
%Curvature
\newcommand{\cg}{\kappa_\mathrm g}
\newcommand{\cn}{\kappa_\mathrm n}
\newcommand{\cspI}{\kappa_{\spI}}
\newcommand{\cspII}{\kappa_{\spII}}

\newcommand{\G}[1]{\Gamma^{\StrChar{#1}{1}}_{\StrChar{#1}{2}\StrChar{#1}{3}}}

\newcommand{\ei}{{\vec e}_i}
\newcommand{\er}{{\vec e}_r}
\newcommand{\ea}{{\vec e}_a}
\newcommand{\eb}{{\vec e}_b}
\newcommand{\eI}{{\vec e}_1}
\newcommand{\eIk}{{\vec e}_{1,k}}
\newcommand{\eIkmI}{{\vec e}_{1,k-1}}
\newcommand{\eIz}{{\vec e}_{1,0}}
\newcommand{\eII}{{\vec e}_2}
\newcommand{\eIIk}{{\vec e}_{2,k}}
\newcommand{\eIII}{{\vec e}_3}
\newcommand{\eIIIk}{{\vec e}_{3,k}}
\newcommand{\eIt}{\tilde{\vec e}_1}
\newcommand{\eIIt}{\tilde{\vec e}_2}
\newcommand{\eIIIt}{\tilde{\vec e}_3}
\newcommand{\eit}{\tilde{\vec e}_i}

\newcommand{\TeI}{\mathcal N_{\eI}}
\renewcommand{\x}{\vec \xi}
\newcommand{\xd}{\vec \xi\d}
\newcommand{\xp}{\dot{\vec \xi}}

%xi i
\newcommand{\xii}{\xi_i}
\newcommand{\xiI}{\xi_1}
\newcommand{\xiII}{\xi_2}
\newcommand{\xiIII}{\xi_3}
\newcommand{\xiIV}{{\xi_4}}
\newcommand{\xiV}{{\xi_5}}
\newcommand{\xiVI}{\xi_6}
\newcommand{\xiVIz}{\xi_{6,0}}
%xi punkt
\newcommand{\xipi}{\dot{\xi}_i}
\newcommand{\xipI}{\dot{\xi}_1}
\newcommand{\xipII}{\dot{\xi}_2}
\newcommand{\xipIII}{\dot{\xi}_3}
\newcommand{\xipIV}{\dot{\xi}_4}
\newcommand{\xipV}{\dot{\xi}_5}
\newcommand{\xipVI}{\dot{\xi}_6}
%xi punkt punkt
\newcommand{\xippi}{\ddot{\xi}_i}
\newcommand{\xippI}{\ddot{\xi}_1}
\newcommand{\xippII}{\ddot{\xi}_2}
\newcommand{\xippIII}{\ddot{\xi}_3}
\newcommand{\xippIV}{\ddot{\xi}_4}
\newcommand{\xippV}{\ddot{\xi}_5}
\newcommand{\xippVI}{\ddot{\xi}_6}
%xi desired i
\newcommand{\xidI}{\xi\d_1}
\newcommand{\xidII}{\xi_2\d}
\newcommand{\xidIII}{\xi_3\d}
\newcommand{\xidIV}{\xi_4\d}
\newcommand{\xidV}{\xi_5\d}
\newcommand{\xidVI}{{\xi\d_6}}

%xi desired punkt
\newcommand{\xidpI}{\dot{\xi}\d_1}

%xi desired punkt punkt
\newcommand{\xidppI}{\ddot{\xi}\d_1}

\newcommand{\xiIk}{\xi_{1,k}}
\newcommand{\xiIkmI}{\xi_{1,k-1}}
\newcommand{\xit}{\vec \xi_\mathrm t}
\newcommand{\xir}{\vec \xi_\mathrm r}
\newcommand{\xirp}{\dot{\vec \xi}_\mathrm r}

\newcommand{\xiR}{{\xi_{r+3}}}
\newcommand{\xiA}{{\xi_{a+3}}}
\newcommand{\xiB}{{\xi_{b+3}}}
\newcommand{\xipR}{{\dot{\xi}_{r+3}}}
\newcommand{\xipA}{{\dot{\xi}_{a+3}}}
\newcommand{\xipB}{{\dot{\xi}_{b+3}}}

\newcommand{\alphaNatural}{\alpha}
\newcommand{\alphaParallel}{\alpha}
\newcommand{\betaNatural}{\beta}
\newcommand{\betaParallel}{\beta}
\newcommand{\gammaNatural}{\gamma}
\newcommand{\gammaNaturali}{\gamma_i}
\newcommand{\gammaNaturalII}{\gamma_2}
\newcommand{\gammaNaturalIII}{\gamma_3}
\newcommand{\gammaParallel}{\gamma}
\newcommand{\gammaParalleli}{\gamma_i}
\newcommand{\gammaParallelII}{\gamma_2}
\newcommand{\gammaParallelIII}{\gamma_3}

\newcommand{\Diffeomorphism}{\vec\Phi}
\newcommand{\TransformationMatrix}{\vec L}

\newcommand{\xie}{\hat{\vec e}}
\newcommand{\xieI}{\hat{e}_1}
\newcommand{\xieIp}{\dot{\hat{e}}_1}
\newcommand{\xieII}{\hat{e}_2}
\newcommand{\xieIIp}{\dot{\hat{e}}_2}
\newcommand{\xieIII}{\hat{e}_3}
\newcommand{\xieIIIp}{\dot{\hat{e}}_3}
\newcommand{\xieIV}{\hat{e}_4}
\newcommand{\xieIVp}{\dot{\hat{e}}_4}
\newcommand{\xieV}{\hat{e}_5}
\newcommand{\xieVp}{\dot{\hat{e}}_5}
\newcommand{\xieVI}{\hat{e}_6}
\newcommand{\xieVIp}{\dot{\hat{e}}_6}


\newcommand{\N}{\mathcal{N}}

\newcommand{\pinv}[1]{{#1}^{\dagger}}
\newcommand{\Ts}{{T_\mathrm s}}
\newcommand{\TsFT}{{T_{\mathrm{s,F/T}}}}
\newcommand*{\subfloatletter}[1]{(#1)}

\newcommand{\mathdirectcurrent}{\mathrel{\mathpalette\mathdirectcurrentinner\relax}}
\newcommand{\mathdirectcurrentinner}[2]{%
  \settowidth{\dimen0}{$#1=$}%
  \vbox to .85ex {\offinterlineskip
    \hbox to \dimen0{\hss\leaders\hrule\hskip.85\dimen0\hss}
    \vskip.35ex
    \hbox to \dimen0{\hss
      \leaders\hrule\hskip.17\dimen0
      \hskip.17\dimen0
      \leaders\hrule\hskip.17\dimen0
      \hskip.17\dimen0
      \leaders\hrule\hskip.17\dimen0
      \hss}
    \vfill
  }%
}
\newcommand{\textdirectcurrent}{\mathdirectcurrentinner{\textstyle}{}}

\providecommand{\Robot}{\Kuka LBR iiwa 14 R820\xspace}
\providecommand{\FTsensor}{\textsc{Ati} Mini 40\xspace}
\providecommand{\EtherCAT}{\textsc{EtherCAT}\xspace}
\providecommand{\TwinCAT}{\textsc{TwinCAT}\xspace}

\providecommand{\Beckhoff}{\textsc{Beckhoff}\xspace}
\providecommand{\Kuka}{\textsc{Kuka}\xspace}
\providecommand{\Newton}{\textsc{Newton}\xspace}
\providecommand{\PicardLindeloef}{\textsc{Picard-Lindelöf}\xspace}
\providecommand{\GramSchmidt}{\textsc{Gram-Schmidt}\xspace}
\providecommand{\Christoffel}{\textsc{Christoffel}\xspace}
\providecommand{\Lagrange}{\textsc{Lagrange}\xspace}
\providecommand{\Euler}{\textsc{Euler}\xspace}
\providecommand{\TaitBryan}{\textsc{Tait-Bryan}\xspace}
\providecommand{\Bernoulli}{\textsc{Bernoulli}\xspace}
\providecommand{\Coriolis}{\textsc{Coriolis}\xspace}
\providecommand{\GoughStewart}{\textsc{Gough-Stewart}\xspace}
\providecommand{\Gauss}{\textsc{Gauss}\xspace}
\providecommand{\GaussCodazzi}{\textsc{Gauss-Codazzi}\xspace}
\providecommand{\DenavitHartenberg}{\textsc{Denavit-Hartenberg}\xspace}
\providecommand{\Iverson}{\textsc{Iverson}\xspace}
\providecommand{\MonteCarlo}{\textsc{Monte-Carlo}\xspace}
\providecommand{\NelderMead}{\textsc{Nelder-Mead}\xspace}
%\providecolor{added}{rgb}{0.9,0,0}
%\newcommand{\changed}[1]{{\color{added}{}#1}}
%\providecolor{deleted}{rgb}{0.6,0.6,0.6}
%\newcommand{\deleted}[1]{{\color{deleted}{}#1}}
%\newcommand{\deleted}[1]{}

\newcommand{\circledAt}[3]{\node[shape=circle,draw,inner sep=1pt] at (axis cs:#2,#3) (char) {\footnotesize #1};}
\DeclareRobustCommand\circled[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=1pt] (char) {\footnotesize #1};}}
\newcommand{\circledAtIII}[4]{\node[shape=circle,draw,inner sep=1pt] at (axis cs:#2,#3,#4) (char) {\footnotesize #1};}

\newcommand{\todo}[1]{ \marginpar{ \textcolor{acin_red}{\begin{spacing}{0.7} \footnotesize #1 \end{spacing}}} }

\newcommand{\videourlI}{\href{https://www.acin.tuwien.ac.at/52f5}{\texttt{www.acin.tuwien.ac.at/52f5}}}
\newcommand{\videourlII}{\href{https://www.acin.tuwien.ac.at/fc09}{\texttt{www.acin.tuwien.ac.at/fc09}}}

\newcommand{\ConceptCategories}[1]{\vspace{-7pt}
  \includegraphics{./graphics/conceptstudy/#1}\\}

\newcommand{\concept}[2]{\hyperref[#2]{\##1}}
\newcommand{\conceptShapeAdaptiveGripper}{\concept{1}{sec:conceptstudy:concepts:shape_adaptive_gripper}\xspace}
\newcommand{\conceptShapeAdaptiveTable}{\concept{2}{sec:conceptstudy:concepts:shape_adaptive_table}\xspace}
\newcommand{\conceptTapeDispenserToolEndeffector}{\concept{3}{sec:conceptstudy:concepts:tape_dispenser_tool_endeffector}\xspace}
\newcommand{\conceptTapeDispenserToolStationary}{\concept{4}{sec:conceptstudy:concepts:tape_dispenser_tool_stationary}\xspace}
\newcommand{\conceptStationaryTapeDispenserLiner}{\concept{5}{sec:conceptstudy:concepts:stationary_tape_dispenser_liner}\xspace}
\newcommand{\conceptStationaryTapeDispenserConveyorbelt}{\concept{6}{sec:conceptstudy:concepts:stationary_tape_dispenser_conveyorbelt}\xspace}
\newcommand{\conceptRollUpTool}{\concept{7}{sec:conceptstudy:concepts:roll_up_tool}\xspace}
\newcommand{\conceptMultiRobotCell}{\concept{8}{sec:conceptstudy:concepts:multi_robot_cell}\xspace}
\newcommand{\conceptAdditiveMethodUnitPatchApplication}{\concept{9}{sec:conceptstudy:concepts:additive_method_unit_patch_application}\xspace}
\newcommand{\conceptAdditiveMethodPrinting}{\concept{10}{sec:conceptstudy:concepts:additive_method_printing}\xspace}

\newcommand{\Concept}[3]{\hyperref[#2]{``#3''}}
\newcommand{\ConceptShapeAdaptiveGripper}{\Concept{1}{sec:conceptstudy:concepts:shape_adaptive_gripper}{Shape-adaptive gripper}\xspace}
\newcommand{\ConceptShapeAdaptiveTable}{\Concept{2}{sec:conceptstudy:concepts:shape_adaptive_table}{Shape-adaptive table}\xspace}
\newcommand{\ConceptTapeDispenserToolEndeffector}{\Concept{3}{sec:conceptstudy:concepts:tape_dispenser_tool_endeffector}{Tape dispenser tool with supply at end-effector}\xspace}
\newcommand{\ConceptTapeDispenserToolStationary}{\Concept{4}{sec:conceptstudy:concepts:tape_dispenser_tool_stationary}{Tape dispenser tool with stationary supply}\xspace}
\newcommand{\ConceptStationaryTapeDispenserLiner}{\Concept{5}{sec:conceptstudy:concepts:stationary_tape_dispenser_liner}{Stationary tape dispenser with liner}\xspace}
\newcommand{\ConceptStationaryTapeDispenserConveyorbelt}{\Concept{6}{sec:conceptstudy:concepts:stationary_tape_dispenser_conveyorbelt}{Stationary tape dispenser with conveyor belt}\xspace}
\newcommand{\ConceptRollUpTool}{\Concept{7}{sec:conceptstudy:concepts:roll_up_tool}{Roll-up tool}\xspace}
\newcommand{\ConceptMultiRobotCell}{\Concept{8}{sec:conceptstudy:concepts:multi_robot_cell}{Multi-robot cell}\xspace}
\newcommand{\ConceptAdditiveMethodUnitPatchApplication}{\Concept{9}{sec:conceptstudy:concepts:additive_method_unit_patch_application}{Unit patch application}\xspace}
\newcommand{\ConceptAdditiveMethodPrinting}{\Concept{10}{sec:conceptstudy:concepts:additive_method_printing}{3D Printing}\xspace}

\newcommand{\CONCEPT}[3]{\hyperref[#2]{\##1 ``#3''}}
\newcommand{\CONCEPTShapeAdaptiveGripper}{\CONCEPT{1}{sec:conceptstudy:concepts:shape_adaptive_gripper}{Shape-adaptive gripper}\xspace}
\newcommand{\CONCEPTShapeAdaptiveTable}{\CONCEPT{2}{sec:conceptstudy:concepts:shape_adaptive_table}{Shape-adaptive table}\xspace}
\newcommand{\CONCEPTTapeDispenserToolEndeffector}{\CONCEPT{3}{sec:conceptstudy:concepts:tape_dispenser_tool_endeffector}{Tape dispenser tool with supply at end-effector}\xspace}
\newcommand{\CONCEPTTapeDispenserToolStationary}{\CONCEPT{4}{sec:conceptstudy:concepts:tape_dispenser_tool_stationary}{Tape dispenser tool with stationary supply}\xspace}
\newcommand{\CONCEPTStationaryTapeDispenserLiner}{\CONCEPT{5}{sec:conceptstudy:concepts:stationary_tape_dispenser_liner}{Stationary tape dispenser with liner}\xspace}
\newcommand{\CONCEPTStationaryTapeDispenserConveyorbelt}{\CONCEPT{6}{sec:conceptstudy:concepts:stationary_tape_dispenser_conveyorbelt}{Stationary tape dispenser with conveyor belt}\xspace}
\newcommand{\CONCEPTRollUpTool}{\CONCEPT{7}{sec:conceptstudy:concepts:roll_up_tool}{Roll-up tool}\xspace}
\newcommand{\CONCEPTMultiRobotCell}{\CONCEPT{8}{sec:conceptstudy:concepts:multi_robot_cell}{Multi-robot cell}\xspace}
\newcommand{\CONCEPTAdditiveMethodUnitPatchApplication}{\CONCEPT{9}{sec:conceptstudy:concepts:additive_method_unit_patch_application}{Unit patch application}\xspace}
\newcommand{\CONCEPTAdditiveMethodPrinting}{\CONCEPT{10}{sec:conceptstudy:concepts:additive_method_printing}{3D Printing}\xspace}


==> graphics/packages.tex <==
\usepackage{xcolor}
\usepackage{siunitx}
% \sisetup{per-mode=symbol,binary-units=true,exponent-product = \cdot}

%\usepackage[nohyperlinks]{acronym}

\usepackage{tikz}


==> graphics/packages_pgfplots.tex <==
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}
\pgfkeys{/pgf/number format/.cd,1000 sep={\,}}
\pgfplotsset{compat=1.12,height=0.3\textheight,legend cell align=left,tick scale binop=\times}
\pgfplotsset{tick style={black,thin}}
\pgfplotsset{every axis plot/.append style={line width=0.8pt}}
% \pgfplotsset{every axis/.append style={line join=round,no markers}}
\pgfplotsset{every axis/.append style={line join=round}}
% \pgfplotsset{legend style={draw=none,fill=white,fill opacity=0.6,text opacity=1}}
\pgfplotsset{ylabsh/.style={every axis y label/.style={at={(0,0.5)}, xshift=#1, rotate=90}}}
\pgfplotsset{
  legend image with text/.style={
    legend image code/.code={%
      \node[anchor=center] at (0.3cm,0cm) {#1};
    }
  },
}

\pgfplotsset{
  cycle list={acin_red,thick\\
    acin_green_variant,thick\\
    TU_blue,thick\\
    TU_violet_variant!80!black,thick\\
    orange!90!white,thick\\
    acin_green!45!TU_blue!90,thick\\
    TU_gray,thick\\
    brown!80!black,thick\\
  }
}

\pgfplotsset{
    colormap={parula}{
        rgb255=(53,42,135)
        rgb255=(15,92,221)
        rgb255=(18,125,216)
        rgb255=(7,156,207)
        rgb255=(21,177,180)
        rgb255=(89,189,140)
        rgb255=(165,190,107)
        rgb255=(225,185,82)
        rgb255=(252,206,46)
        rgb255=(249,251,14)
    },
}


==> tex/rel_err_stat.tex <==
\begin{tabular}{l c c}
           & $\norm{\tilde{\vec{e}}_t}$    & $\tilde{\Theta}_r$                    \\ \hline
Mean       & \SI{0.0253}{\milli \m} (\SI{0.00194}{\percent})      & \SI{0.661}{\degree}   \\
Std. Dev.  & \SI{1.37}{\milli \m} (\SI{0.105}{\percent})      & \SI{0.314}{\degree}   \\
Maximum    & \SI{4.91}{\milli \m} (\SI{0.377}{\percent})      & \SI{1.97}{\degree}   \\ \hline
\end{tabular}

